L2CU: Learning to Complement Unseen Users

Recent research highlights the potential of machine learning models to learn to complement (L2C) human strengths; however, generalizing this capability to unseen users remains a significant challenge. Existing L2C methods oversimplify interaction between human and AI by relying on a single, global user model that neglects individual user variability, leading to suboptimal cooperative performance. Addressing this, we introduce L2CU, a novel L2C framework for human-AI cooperative classification with unseen users. Given sparse and noisy user annotations, L2CU identifies representative annotator profiles capturing distinct labeling patterns. By matching unseen users to these profiles, L2CU leverages profile-specific models to complement the user and achieve superior joint accuracy. We evaluate L2CU on datasets (CIFAR-10N, CIFAR-10H, Fashion-MNIST-H, Chaoyang and AgNews), demonstrating its effectiveness as a model-agnostic solution for improving human-AI cooperative classification.

==> tables/experiments/ex_abl_users.tex <==
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{colortbl}
% \usepackage{hhline}


% \begin{table}
% \centering
% \arrayrulecolor{black}
% \resizebox{\linewidth}{!}{%
\begin{tabular}{lc|ccccccccccc} 
\hline
\multirow{2}{*}{Dataset} & \multirow{2}{*}{Users} & \multicolumn{3}{c}{K=1} & ~ & \multicolumn{3}{c}{K=2} & ~ & \multicolumn{3}{c}{K=3} \\ 
\cline{3-13}
 &  & I & S & NI & ~ & I & S & NI & ~ & I & S & NI \\ 
\hhline{>{\arrayrulecolor{black}}==>{\arrayrulecolor{black}}===========}
~ & \multicolumn{1}{c}{~} & \multicolumn{11}{c}{With simulated annotators} \\ 
\hline
\multirow{2}{*}{CIFAR10} & 15 & 5 & 0 & 10 &  & 9 & 0 & 6 &  & 15 & 0 & 0 \\
 & {\cellcolor[rgb]{0.949,0.949,0.949}}15 & {\cellcolor[rgb]{0.949,0.949,0.949}}5 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}10 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}9 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}6 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}15 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-13}
\multirow{2}{*}{AgNews} & 15 & 15 & 0 & 0 &  & 15 & 0 & 0 &  & 15 & 0 & 0 \\
 & {\cellcolor[rgb]{0.949,0.949,0.949}}15 & {\cellcolor[rgb]{0.949,0.949,0.949}}15 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}15 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}15 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-13}
~ & \multicolumn{1}{c}{~} & \multicolumn{11}{c}{With real annotators} \\ 
\hline
\multirow{2}{*}{CIFAR10-N} & 80 & 80 & 0 & 0 &  & 80 & 0 & 0 &  & 80 & 0 & 0 \\
 & {\cellcolor[rgb]{0.949,0.949,0.949}}80 & {\cellcolor[rgb]{0.949,0.949,0.949}}80 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}80 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}80 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-13}
\multirow{2}{*}{CIFAR10-H} & 2571 & 2548 & 0 & 23 &  & 2566 & 1 & 4 &  & 2567 & 1 & 3 \\
 & {\cellcolor[rgb]{0.949,0.949,0.949}}2022 & {\cellcolor[rgb]{0.949,0.949,0.949}}2022 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}2022 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}2022 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-13}
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Fashion-\\MNIST-H\end{tabular}} & 183 & 182 & 0 & 1 &  & 183 & 0 & 0 &  & 183 & 0 & 0 \\
 & {\cellcolor[rgb]{0.949,0.949,0.949}}182 & {\cellcolor[rgb]{0.949,0.949,0.949}}182 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}182 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}182 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-13}
\multirow{2}{*}{Chaoyang} & 3 & 2 & 0 & 1 &  & 2 & 0 & 1 &  & 3 & 0 & 0 \\
 & {\cellcolor[rgb]{0.949,0.949,0.949}}2 & {\cellcolor[rgb]{0.949,0.949,0.949}}2 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}2 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}~ & {\cellcolor[rgb]{0.949,0.949,0.949}}2 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 & {\cellcolor[rgb]{0.949,0.949,0.949}}0 \\
\hhline{>{\arrayrulecolor{black}}->{\arrayrulecolor{black}}------------}
\end{tabular}
% }
% \arrayrulecolor{black}
% \end{table}
